Mobility for Cellular-Connected UAVs: challenges for the network provider

Unmanned Aerial Vehicle (UAV) technology is becoming more prevalent and more diverse in its application. 5G and beyond networks must enable UAV connectivity. This will require the network operator to consider this new type of user in the planning and operation of the network. This work presents the challenges an operator will encounter and should consider in the future as UAVs become users of the network. We analyse the 3GPP specifications, the existing research literature, and a publicly available UAV connectivity dataset, to describe the challenges. We classify these challenges into network planning and network optimisation categories. We discuss the challenge of planning network coverage when considering coverage for flying users and the PCI collision and confusion issues that can be aggravated by these users. In discussing network optimisation challenges, we introduce Automatic Neighbouring Relation (ANR) and handover challenges, specifically the number of neighbours in the Neighbour Relation Table (NRT), and their potential deletion and block-listing, the frequent number of handovers and the possibility that the UAV disconnects because of handover issues. We discuss possible approaches to address the presented challenges and use a real-world dataset to support our findings about these challenges and their importance.

==> biography.tex <==

%\begin{IEEEbiographynophoto}{Luiz A. DaSilva}
%  holds the Telecommunications chair at TCD,
%  where he is the director of CONNECT.
%\end{IEEEbiographynophoto}

%\vfill


==> sections/related.tex <==
\section{State of the art}
\label{sec:related}
% !TEX root = ../../main.tex
\erika{Intro to the section}
\ac{son} was introduced in \ac{lte} with intention of optimise some networks procedures, and one of the biggest changes was into the \ac{ue} mobility. \ac{son} introduced \ac{anr}, that has as the principal objective automatically adapt the \ac{nrt} using ue measurements. In 5G, the concept of the \ac{anr} and handover does not differ much to the developed in LTE, although the newer generation introduces a variety of lists types (relations between beams, and relations between a base station and beams, for example) and new users, as \ac{iot} and \acp{uav}. The detailed explanation of ANR and handover is described in \cite{3GPP_2019}. This section will introduce how previous works deal with handover management after the implementation of \ac{anr} in \ac{lte} and how the research community is approaching the challenge for 5G networks.%cellular-connected UAV. 



%I still need to figure out if I will explain ANR and in which detail
\erika{first works in ANR}
One of the first works on optimisation in \acp{anr} was presented in \cite{firsts-anr}. Authors proposed a distributed approach, where each \ac{bs} checks with the around \acp{bs} the set of \acp{ue} and their service area. If the intersected set is larger than a threshold, the BS is added to the \ac{anr}. It is a way to check the coverage area of its neighbours using the service area it has at all the moments. For this procedure to be up to date, it needs to be executed periodically, causing overhead in the signalling of the network and also, assumes that the neighbours will be near to each other, what might not happen for connected \acp{uav} as it has a bigger chance to connect to further \acp{bs} \cite{qualcom}. 

In \ac{pingpong} authors analyse the handover probabilities considering an hexagonal structure. In this scenario, the NRT would contain the 6 closest \acp{bs}. They assume 2 channels, 1 for control and one for data (as 5G for small cells). On their assumptions, there is no way a target BS is not on the NRT. They use Markov probabilities to check the chances of moving to a neighbour BS, and based on this probability, they predict the next BS the \ac{uav} will connect to. They managed to reduce the delay of the handovers in \textcolor{red}{I WILL ADD IT}. This solution would have escalated issues once applied to the \ac{uav} reality, where it senses far away \acp{bs}. The Markov decisions would increase complexity once the number of possible \ac{bs} increase.

\erika{they point out the importance of less signalling and need to identify new neighbours for 5G}
In \cite{ramachandra2016automatic}, authors present the \ac{anr} for LTE, and how it has to improve to attend 5G requirements. It brings out a new challenge that is the ultra-lean design, where the cellular  network has to save energy as much as possible, avoiding unnecessary control messages and measurements. 
It discusses the need for alternatives types of identifier and neighbours relations for 5G. It does not study the problem on the point of view of the new types of user that 5G brings, although, explain the general relationships need in 5G.

\erika{Predicting Ho, based on planned NR - not actualised not for 5g}
In \cite{mohamed2018memory}, authors propose a memory-full context-aware \ac{ho} procedure for 5G networks that perform mobility prediction to avoid unnecessary signalling messages. The proposed scheme predict the \ac{ho} events in the future with expected \acp{ho} times, using information of \ac{ue} history of \ac{ho}, \ac{bs}'s \acp{nrt}, speed and direction. With the prediction, they perform the handover signalling in advance, and propose to the \ac{ue} do not make more periodically measurements reports. Their results show a promising direction to avoid unnecessary mobility signalling. Although their solution is promising, it does not take in consideration the type of user that is performing the \ac{ho} neither its height, so the coverage expected area of the \acp{bs} are easier to predict as it is made for the \ac{gue}. They use statistics applied to the \ac{nrt} of the source \ac{bs}, so for \acp{uav} the distant \ac{bs} that they might connect would not be on the list, which could result on not to choose the best serving \ac{bs} or even to disconnecting time. 
%The main challenge add by the connected \acp{uav} is the unpredictable aerial coverage that could affect their prediction model. 

\erika{Ranking work}
In \cite{gorccin2017hybrid}, authors propose comprehensive hybrid ANR (H-ANR) architecture that makes the management of the relations between \acp{bs} based on performance criteria, \ac{ue} measurements and configuration metrics. They propose a ranking of the neighbours based on the distance to the \acp{bs}, historical values of their performance and avoiding \acp{bs} that have a significant number of \ac{hof}, also using the concept of priority-listing and block-listing.
As they use the distance of the \ac{bs}, in the criteria to rank the \ac{anr} this ranking would not be assertive to connected \acp{uav} as the best signal might come from further \acp{bs}.





==> sections/result.tex <==
\section{Experimental prove of concept}
\label{sec:result}
To support that the UAV should be considerate on the various steps of the network planning and configuration, we run an experiment with a mobile phone attached to a UAV and record it's \acp{kpi}. The mobile phone is a Google Pixel 3, and the UAV is a DJI Matrice M300. The network is a 2 tier mobile network in Dublin city centre that operates on the 3.6GHz. The results in this paper will only evaluate the small-cell deployment. The operator uses a parameter that gives preference to the ue to be connected on the small-cells. 

At this experiment, the UAV was flying above the River Liffey, making the same horizontal path and varying its height. %, as shown in Figure \ref{fig:liffey}. The blue circles on the image represent the position of the small-cells deployments. On the results, few more small cell are further away into the left of the image and surprisingly provided the connection to the UAV during some times of the experiment. 
The experiment's primary purpose is to check how the \acp{kpi} vary once we vary height in a small-cell deployment. 
%More details on the experiment is presented in \cite{experiment}.

\begin{figure}
  \includegraphics[width=\linewidth]{images/Screenshot.png}
    \caption{3D signal traces of the measured signal strength at different UAV heights along the flight area.}
    \label{fig:liffey}
\end{figure}

Usually, for \ac{gue} it is a fair assumption that the ue will be connected to the closest \ac{gnb}, being this common in the research community to assume \cite{boris paper +other - Boris, can you help?}. In this first analyses, we analyse how often the UAV was connected to the closest \ac{gnb}. Figure \ref{fig:closest} illustrates how often the UAV connects to the closest \ac{gnb} and further \ac{gnb}s for four different altitudes, 30m, 60m, 90m and 120m. At 30m, the UAV connects more often to the closest \ac{gnb}, which does not happen to the higher altitudes. When the UAV is at 120m it spends most of the time connected to the fourth furthest \ac{gnb}s and during all different altitudes, it spend some times connected to a 5th or more distant \ac{gnb}s. The behaviour presented on the results differs from a expected behaviour from a \ac{gue}.  

Results showed in \ref{fig:closest} reinforce the idea that the air planning coverage needs to be considered before deploying new \ac{gnb}s, as the UAVs do not behave as \ac{gue} and can connect to much further \ac{gnb}s. It also draws attention to the research community's assumptions that the UAV connects to its closest \ac{gnb}s is not what happens in reality for at least 46\% of the time. 

\begin{figure}
  \includegraphics[width=\linewidth]{images/distance_to_bs.png}
    \caption{Percentage of time the UAV was connected to the BSs based on its distance.}
    \label{fig:closest}
\end{figure}

Another interesting study on the small-cell deployment is the ping-pong effect on the UAV once flying through the network. Figure \ref{fig:pingpong} illustrates how often the UAV performed ping-pong %, which means did a handover to a cell and come back to the last cell 
in a short period (less than 2s). The results show that the biggest height provides the biggest number of ping-pongs. At 90m the UAV had slightly fewer ping-pongs then at the height of 60m. We believe that to understand the dynamics of the ping-pong effect on UAVs, it needs further investigation. The planning tools considering side-lobes and the air coverage will help the research community evaluate these results.
These results show that the network configuration can be better adequate for the UAVs to start event A3 that generates the handover.

\begin{figure}
  \includegraphics[width=\linewidth]{images/ping-pong.png}
    \caption{Number of ping-pong handovers during the path per altitude.}
    \label{fig:pingpong}
\end{figure}



